Hardness of Approximation in P via Short Cycle Removal: Cycle Detection, Distance Oracles, and Beyond

We present a new technique for efficiently removing almost all short cycles in a graph without unintentionally removing its triangles. Consequently, triangle finding problems do not become easy even in almost $k$-cycle free graphs, for any constant $k\geq 4$. Triangle finding is at the base of many conditional lower bounds in P, mainly for distance computation problems, and the existence of many $4$- or $5$-cycles in a worst-case instance had been the obstacle towards resolving major open questions. Hardness of approximation: Are there distance oracles with $m^{1+o(1)}$ preprocessing time and $m^{o(1)}$ query time that achieve a constant approximation? Existing algorithms with such desirable time bounds only achieve super-constant approximation factors, while only $3-\epsilon$ factors were conditionally ruled out (P\u{a}tra\c{s}cu, Roditty, and Thorup; FOCS 2012). We prove that no $O(1)$ approximations are possible, assuming the $3$-SUM or APSP conjectures. In particular, we prove that $k$-approximations require $\Omega(m^{1+1/ck})$ time, which is tight up to the constant $c$. The lower bound holds even for the offline version where we are given the queries in advance, and extends to other problems such as dynamic shortest paths. The $4$-Cycle problem: An infamous open question in fine-grained complexity is to establish any surprising consequences from a subquadratic or even linear-time algorithm for detecting a $4$-cycle in a graph. We prove that $\Omega(m^{1.1194})$ time is needed for $k$-cycle detection for all $k\geq 4$, unless we can detect a triangle in $\sqrt{n}$-degree graphs in $O(n^{2-\delta})$ time; a breakthrough that is not known to follow even from optimal matrix multiplication algorithms.

==> intro-amir.tex <==

One of the most central and challenging goals in fine-grained complexity is to prove \emph{hardness of approximation} results for the many fundamental problems that we already know are hard to compute exactly.
With the exception of few results that follow from simple gadget reductions,\footnote{Similar to saying that the NP-hardness of $3$-coloring implies a $4/3-\eps$-hardness of approximation for the chromatic number.} understanding the time vs. approximation tradeoff seems to require specialized fine-grained \emph{gap amplification} techniques.
As we know from the quest for \emph{NP-hardness} of approximation that started in the early 90's, such techniques are not easy to come by, and the fine-grained restrictions on the reductions can only make matters worse.

Two notable success stories, highlighted in a recent survey by Rubinstein and Vassilevska Williams \cite{RVsurvey}, are the Distributed PCP framework \cite{ARW17} based on algebraic error-correcting codes, and a graph-products technique \cite{B+21} that has lead to impressive lower bounds for the Diameter problem \cite{DVVW19,Bonnet21a,Li21,DW21,Bonnet21b,DLV21}.
But we are still far away from satisfactory results for many problems (see the open questions in \cite{ARW17,RVsurvey}).
Even \emph{distance computations in graphs}, an extensively studied subject in fine-grained complexity, exhibits many huge gaps. 

As a case in point, consider the open questions below for three of the most basic problems in the area, each of them with a long list of upper bounds (summarized in Tables 1,2,3): distance oracles \cite{PR14,PRT12,3,4,5,6,7,8,9,10}, dynamic shortest paths \cite{1,2,3,4,5,6,7,8,9,10}, and the girth \cite{1,2,3,4,5,6,7,8,9,10}.


\begin{oq}
Can we preprocess a graph in $m^{1+o(1)}$ time and answer shortest path queries in $m^{o(1)}$ time with an $O(1)$-approximation? How about a much better, $3$-approximation?
\end{oq}

\begin{oq}
Can we preprocess a graph in $O(mn)$ time, then support edge-updates in $m^{o(1)}$ amortized time, and answer shortest path queries in $m^{o(1)}$ time with an $O(1)$-approximation? How about a $2$-approximation?
\end{oq}


\begin{oq}
Can we return an $O(1)$-approximation to the girth in $m^{1+o(1)}$ time? How about a $4/3$-approximation?
\end{oq}

The current upper bounds have the form of $O(k)$-approximation in $\tilde{O}(m^{1+1/k})$ time, meaning that only super-constant approximation factors are possible in $m^{1+o(1)}$ time.
It seems plausible that this is the right tradeoff, but it is hard to be confident without a hardness result. 
Such a tradeoff curve was recently broken, in an equally unexpected manner, for the Edit Distance problem \cite{BEGHS21,CDG+20,AN20}. 

Meanwhile, the lower bounds are consistent with positive answers to \emph{all} of these questions, even in \emph{weighted} graphs.\footnote{The case of \emph{directed} graphs is different however. For some of these problems even deciding if the distance is finite has strong lower bounds.}
Existing techniques cannot even rule out small (constant) approximation factors.

The barrier for proving higher lower bounds is common; it is the \emph{short cycle barrier} discussed below.
Overcoming this barrier is related to Open Question 5 in the distributed PCP paper \cite{ARW17} asking for gap amplification techniques from conjectures other than SETH.
This is because (the exact versions of) our distance computation problems are not SETH-hard; their hardness is via  reductions from (detecting or) \emph{listing triangles} in a graph, a problem that is hard under the 3SUM or APSP conjectures, but not SETH.



\paragraph{The Short Cycle Barrier.}
Suppose we are given a tripartite graph $G$ with parts $A,B,C$ and want to detect a triangle $a\in A, b \in B, c \in C$.\footnote{This tripartite version is equivalent to the general case by a standard reduction.}
Let $G'$ be the graph obtained from $G$ by removing the $B \times C$ edges.
For each pair $(b,c) \in E(G)$, what is the distance between $b$ and $c$ in $G'$?
It is $2$ if $(b,c)$ is in a triangle in $G$, and larger otherwise. 
But how much larger?
Unfortunately from a hardness of approximation perspective, the distance will probably not be more than $4$ due to a path with one \emph{zigzag}  $b \to a \to b' \to a' \to c$  that corresponds to a $5$-cycle in $G$ but not a triangle.
So we cannot go above $(2-\eps)$ factors in this way.

In FOCS 2010, P{\u{a}}tra{\c{s}}cu and Roditty \cite{PR14} devised an ingenious graph-products technique (that was an inspiration for the Diameter results \cite{B+21}) to push the lower bound beyond $2$.
The idea was to have a construction with $k$ layers such that a pair $b,c$ without a direct path (of length $k$) must make a zigzag in $k-1$ layers, making the distance $3k-2$.
Indeed, this was accomplished in a follow-up paper with Thorup \cite{PRT12} that went all the way up to $(3-\eps)$ factors, but it is clear that this is the limit of the approach. 

The natural and more promising approach for circumventing this barrier is to simply assume that there are no $\leq k$-cycles in the graph. 
Then, any effective zigzag must be \emph{long}, and even with the natural two-layered construction, would give us a lower bound of $\Omega(k)$.
Indeed, the distance for a pair $b,c$ would be $=2$ if the pair is in a triangle, versus $\geq k-1$ otherwise.
This would be reminiscent of the use of the girth conjecture in lower bounds for \emph{multiplicative} spanners \cite{PS89,Alt+93},
whereas the aforementioned graph-products technique is reminiscent of lower bounds for \emph{additive} spanners \cite{Woodruff06,AB17,ABP18}.\footnote{The Girth Conjecture and the techniques for additive spanners were already used, of course, for lower bounds against distance oracles as well. However, such lower bounds (and any information-theoretic arguments) cannot prove lower bounds higher than $m$; rather, they are interesting for understanding how much dense graphs can be compressed. Thus, the similarity can only be spiritual.}
All we have to do is to prove this gap amplification result for Triangle, amplifying the no-case from triangle-free to $\leq k$-cycle free.


\begin{oq}[Main Open Question]
\label{oq:main}
Can we prove hardness for finding a triangle in a $4$-cycle free graph? What if it is $k$-cycle free for all $k=O(1)$?
\end{oq}

Any progress on this question carries over to progress on the above questions, by the standard reductions.
But it is far from clear why such a gap amplification should be possible.
The needle-in-a-haystack flavor (and intuitive hardness) of triangle finding \emph{stems} from the possibility of a triangle hiding amidst plenty of $4$- or $5$-cycles.
In a $4$-cycle free graph no two nodes can have more than one common neighbor; doesn't that restrict the search space by too much?\footnote{Such high-girth assumptions can indeed reduce the complexity of some problems from almost-quadratic to almost-linear. In particular, in the Orthogonal Vectors problem with dimension $d=n^{o(1)}$ (at the core of the Diameter lower bounds, and many others), if no two vectors can have two coordinates that are non-zero, there is an $O(n d^2)$ algorithm.}

These contemplations touch upon a well-known hole in our understanding of graph problems. 
Indeed, by a simple reduction, proving such an amplification even if only for $k=4$ already resolves one of the most infamous open questions in fine-grained complexity:\footnote{By a simple trick where we subdivide a subset of the edges.}

\begin{oq}
Can we determine if a graph contains a $4$-cycle in $m^{1+o(1)}$ time?
\end{oq}

In 1994, Yuster and Zwick \cite{YZ97} put forth the conjecture that one cannot detect a $4$-cycle in a graph in subquadratic time. 
The longstanding upper bound is $O(m^{4/3})$ via a high-degree low-degree argument \cite{AYZ97}; it is at most $O(n^2)$ because when $m \geq 200\cdot n^{1.5}$ we can simply output ``yes'': by the Bondy-Simonovitz Theorem \cite{BS74}, a graph with such density must contain a $4$-cycle.
Frustratingly, to this date, the field of fine-grained complexity has not managed to show any hardness for this problem.
``\emph{What hope do we have to
understand more complex problems if we cannot settle the complexity of this simple one, even
conditionally?}''\footnote{This is a quote from the survey by Rubinstein and Vassilevska Williams \cite{RVsurvey} where it is referring to the approximability of the graph diameter problem. We find it no less poignant when considering the $4$-cycle problem.}

In this paper we answer all of the above questions, some fully and some partially, under plausible hardness assumptions.
Our main contribution is a proof that triangle finding remains hard when the graph has very few short cycles. 


\subsection{First Result: Removing Most $k$-Cycles}


\begin{restatable}{theorem}{ThmRemovingCycles}[Removing Most $k$-Cycles]
\label{thm:main1}
Let $\eps',\eps>0$ and $k\geq 4$. Given a graph $G$ with maximum degree $\sqrt{n}$, for every $\alpha>0$, there is a randomized $O(n^{2-\eps})$-time algorithm that returns a subset of the edges $E' \subseteq E$ with an aswer to each edge $e\in E'$ to whether it participates in a triangle, and a set of $s=n^{3/2-3\alpha}$ subgraphs $G_1,\ldots,G_s$ such that:
\begin{itemize}
    \item If an edge $e \in E$ is in a triangle in $G$ then it is either in $E'$ or is in a triangle in one of the $G_i$'s.
    \item Each $G_i$ has $n^{1/2+\alpha}$ nodes of degree $n^{\alpha}$ with high probability, and contains only $O(n^{\frac{\omega-1}{4}+\eps'+k\alpha})$ $k$-cycles in expectation.
\end{itemize}
\end{restatable}

The problem of reporting which edges in a graph are in a triangle (All-Edge Triangle) is known to require $n^{2-o(1)}$ time, under the $3$-SUM Conjecture \cite{Pat10,KPP16} or under the APSP Conjecture~\cite{VX20}, and this holds even for graphs of degree $\sqrt{n}$.
Thus it is a very plausible conjecture that $n^{2-o(1)}$ is required.

Combining our new theorem with the standard reductions already resolves some of the hardness of approximation problems above. 
Each of the few remaining short cycles might result in a false positive, but since their number is small (and the degrees in the $G_i$ graphs are small), they can all be filtered in post-processing stage of subquadratic time.


\paragraph{Applications}
Our first corollary improves the $(3-\eps)$ hardness of P{\u{a}}tra{\c{s}}cu, Roditty, and Thorup \cite{PRT12} all the way up to $\omega(1)$ showing that $O(k)$-approximation with $\tilde{O}(m^{1+1/k})$ preprocessing is indeed the right tradeoff for distance oracles.\footnote{One caveat is that their lower bound is based on a set-intersection conjecture that rules out preprocessing with $m^{1+\eps}$ \emph{space} rather than \emph{time}, and is therefore stronger. On the other hand, our lower bound is based on the more popular 3SUM and APSP conjectures.}
Moreover, our lower bound applies to the easier \emph{offline} version of the problem where all the queries are given in advance.
 
\begin{corollary}[Hardness of Approximation for Offline Distance Oracles]
Assuming either the $3$-SUM or APSP Conjectures, no algorithm can return a $k$-approximation to the distance between $m$ pairs of nodes in a simple graph with $m$ edges in time $O(m^{1+1/4k-\eps})$\Atodo{todo}, where $\eps>0$.
\end{corollary}

The \emph{Subset Shortest Paths} problem in the above corollary is at the core of the dynamic shortest paths problem as well. 
By a straightforward reduction it implies that Chechik's decremental APSP $k$-approximation algorithm in total time $m^{1+1/ck}$\Atodo{todo} is tight up to the constant $c$.
For fully dynamic algorithms, we can strengthen the result further by ruling out algorithms that start with a cubic-time preprocessing phase (which is natural as it gives the algorithm enough time to precompute all the distances). However, in this fully dynamic case, the best known upper bound only achieves a $(\log{n})^k$-approximation in $m^{1+1/k}$ time.

\begin{corollary}[Hardness of Approximation for Dynamic APSP]
Assuming either the $3$-SUM or APSP Conjectures, no algorithm can preprocess a simple graph in $O(n^3)$ time and then support updates and queries in $O(m^{1/4k-\eps})$ time, for some $\eps>0$, where an answer to a query is a $k$-approximation to the distance between a given pair of nodes. \Atodo{todo: time bounds}
\end{corollary}

\Atodo{Not sure if it's better to include this third application or omit it. }
And as a third corollary, we show that any algorithm that obtains a $k$-approximate shortest cycle for each edge in the graph must spend $m^{1+1/ck}$ time.

\begin{corollary}[Hardness of Approximation for All-Edge Shortest Cycle]
Assuming either the $3$-SUM or APSP Conjectures, no algorithm can return a $k$-approximation to the shortest cycle that each edge is a part of in a simple graph with $m$ edges in time $O(m^{1+1/2k-\eps})$\Atodo{todo}, where $\eps>0$.
\end{corollary}

%This matches a very recent upper bound tradeoff for the girth. Alas, that algorithm does not solve the All-Edge version.


Let us now turn our attention back to the intriguing $4$-Cycle problem.
A direct corollary of our theorem is that the All-Edge version has a super-linear lower bound, finally extending the $m^{4/3}$ lower bound from P{\u{a}}tra{\c{s}}cu's seminal paper \cite{Pat10} for triangle enumeration to a hardness result for $4$-cycle enumeration.
If $\omega=2+o(1)$ the lower bound is $m^{5/4-o(1)}$.

\begin{restatable}[Hardness for $4$-Cycle Enumeration]{corollary}{CorEnum}\label{cor:Enum}
Assuming either the $3$-SUM or APSP Conjectures, no algorithm can process an $m$ edge graph in $O(m^{1+\frac{3-\omega}{2(4-\omega)}-\eps})$ time, for some $\eps>0$, and then enumerate $4$-cycles with $m^{o(1)}$ delay. \Atodo{it might make more sense to say this theorem for all $k \geq 4$ and change the text below.}
\end{restatable}

We can also derive super-linear $m^{1+1/ck}$ lower bounds for $k$-cycle enumeration for all $k$, from Theorem~\ref{thm:main1}. 
However, we can get a higher $m^{5/4-o(1)}$ lower bound by reducing from $4$-Cycle directly: 
simple gadget reductions prove that $k$-cycle (detection or enumeration) for any $k$ is at least as hard as hard as either the $k=3$ or $k=4$ case (see \cite{DKS17}).\footnote{The reduction simply subdivides some of the edges. Note that this trick is not useful in the hardness of approximation context because subdividing edges increases the distances even in the yes-case.} 
Either way, we separate $k$-cycle from the class $\textsc{DelayC}_{lin}$ of problems solvable with linear time preprocessing and constant delay. 
This class has received a lot of attention in recent years from the enumeration algorithms community (see e.g. \cite{1,2,3,4,5}).
Our result is somewhat surprising because enumerating all cycles (without restricting $k$) is \emph{in} the class $\textsc{DelayC}_{lin}$ \cite{sodapaper}.

\medskip
Theorem~\ref{thm:main1} does not fully resolve the Main Open Question~\ref{oq:main}, because it does leave $n^{\Omega(1)}$ short cycles in the graph.
This is not an issue for all of the applications above because the end-problem returns multiple answers (that can be filtered afterwards).
Unfortunately, this cannot be done for problems with a single output, such as our most basic $4$-Cycle detection problem.
Nonetheless, with a bit more work we can actually get rid of all $k$-cycles in the $k=4$ case.
 



%
%This matches a very recent upper bound tradeoff for the girth. Alas, that algorithm does not solve the All-Edge version.
%To prove a similar lower bound for the more basic girth problem, our gap amplification must get rid of \emph{all} $\leq k$-cycles.
%Unfortunately, Theorem~\ref{thm:main1} does leave $n^{\Omega(1)}$ short cycles (and therefore does not fully resolve the Main Open Question~\ref{oq:main}).
%Nonetheless, with a bit more work we can actually get rid of all $k$-cycles in the $k=4$ case.
%
%\Stodo{Something about this paragraph above doesn't feel incredibly good to me. Let's discuss when we meet. See also my second comment below.}

\subsection{Second Result: Removing \emph{all} $4$-Cycles}

Our most technical result is a strengthening of Theorem~\ref{thm:main1} in the $k=4$ case, giving a reduction to graphs that are \emph{completely} $4$-cycle free, finally establishing a conditional lower bound for $4$-Cycle.

\begin{restatable}{theorem}{ThmAllFourCycles}
\label{thm:main2}
Let $\eps>0$ and $0<\alpha<1/4-\frac{\omega-1}{8}-\eps/2$. Given a graph $G$ with maximum degree $\sqrt{n}$, there is a randomized $O(n^{2-\eps})$-time algorithm that returns a subset of the edges $E' \subseteq E$ with an answer for each $e\in E'$ to whether it participates in a triangle, and a set of $s=n^{3/2-3\alpha}$ subgraphs $G_1,\ldots,G_s$ such that:
\begin{itemize}
    \item If an edge $e \in E$ is in a triangle in $G$ then it is either in $E'$ or is in a triangle in one of the $G_i$'s.
    \item  With constant probability, each $G_i$ has $n^{1/2+\alpha}$ nodes of degree $n^{\alpha}$, and is $4$-cycle free.
\end{itemize}
\end{restatable}



\begin{restatable}[Hardness for $4$-Cycle Detection]{corollary}{CorFourDet}\label{cor:fourDet}
Assuming that triangle detection in graphs with maximum degree $\sqrt{n}$ requires $n^{2-o(1)}$ time, no algorithm can determine if an $m$-edge graph has a $4$-cycle in $O(m^{1+\frac{3-\omega}{2(5-\omega)}-\eps})$ time, for some $\eps>0$.
\end{restatable}


The longstanding upper bound for triangle detection is $O(\min\{m^{2\omega/(\omega+1)},n^{\omega}\})$, where $\omega\geq 2+o(1)$ is the fast matrix multiplication exponent \cite{YZ?}.
Even if an optimal matrix multiplication algorithm exists ($\omega=2$) no algorithm breaks the quadratic barrier when $m=n^{1.5}$.
This continues to be the case in the natural setting where the maximum degree (rather than the average degree) is $\sqrt{n}$.
Thus, breaking the hardness assumption at the base of our conditional lower bound would be a major breakthrough.
See Section~\ref{sec:discussion} for further discussion.

In fact, even for triangles, the 3SUM hardness from P{\u{a}}tra{\c{s}}cu's seminal paper \cite{Pat10} (and the later APSP hardness \cite{VX20}) are only known for the enumeration (or \emph{All-Edge} versions) but not for detection.
We show that the same kind of hardness carries over to $4$-cycle.

\begin{restatable}[Hardness for $4$-Cycle Enumeration]{corollary}{CorEnum}\label{cor:Enum}
Assuming either the $3$-SUM or APSP Conjectures, no algorithm can process an $m$ edge graph in $O(m^{1+\frac{3-\omega}{2(4-\omega)}-\eps})$ time, for some $\eps>0$, and then enumerate $4$-cycles with $m^{o(1)}$ delay.
\end{restatable}


\Stodo{Shouldn't we put this after Theorem 1.6? It follows from 1.6 already. To make the twist in the plot that you want for introducing the most technical result, instead of playing on the girth approx challenge, we can play on the 4-cycle detection and cycles classification challenge (with Unfortunately and then Nonetheless, to built it up in a similar way to what you are doing with the all-edge short cycle thing). Then, we add more consequences for girth approximation and hardness of Triangles in 4-cycle free graphs. To be honest I'm not completely sure about the all-edge short cycle problem.. it feels to me that we are selling it in a strange way as we compare it with an upper bound for an easier problem, computing the girth. If I understand correctly, you want to use it because it helps with this nice build up in the intro, which I feel we can do with 4-cycle detection and cycle classification challenge.}
\Atodo{I agree. That's a good idea. I was trying to keep the focus on approximation problems, but it's inevitable to break the focus at some point because we want to present the other results as well... I'll make the change soon.}
Gadget reductions prove that $k$-cycle (detection or enumeration) for any $k$ is at least as hard as hard as either the $k=3$ or $k=4$ case (see \cite{DKS17}). 
In the parlance of the enumeration algorithms literature, we separate $k$-cycle from the class $\textsc{DelayC}_{lin}$ of problems solvable with linear time preprocessing and constant delay.
This is somewhat surprising because enumerating all cycles (without restricting $k$) is in $\textsc{DelayC}_{lin}$ \cite{sodapaper}.

The lower bound for $4$-Cycle follows from the following corollary, giving a positive answer to the $k=4$ case in the Main Open Question~\ref{oq:main}.


\begin{restatable}[Hardness for Triangle in $4$-Cycle-Free Graphs]{corollary}{CorFourFree}\label{cor:fourFree}
Assuming that triangle detection in graphs with degree $\sqrt{n}$ requires $n^{2-o(1)}$ time, no algorithm can determine if an $m$-edge $4$-cycle free graph has a triangle in $O(m^{1+\frac{3-\omega}{2(5-\omega)}-\eps})$ time, for some $\eps>0$.
\end{restatable}


Consequently, we improve the lower bound for the basic girth approximation problem from $4/3-\eps$ to $5/3-\eps$. 

\subsection{Related Work}

The approximating APSP without scaling paper, and Zwick's $(1+\eps)$-APSP. It's worth discussing other approximation results for APSP such as DHZ.

Other hardness of approximation results in P, e.g. for directed shortest cycle by Mina and Virginia \cite{DV21}, and the results that follow from Distributed PCPs. Maybe also the approximate counting results by Dell et al.

Other hardness of approximation for distance computation problems, and other open questions, e.g. $(1+\eps)$ dynamic APSPS in planar.

Lower bounds for $4$-cycle in other settings (directed, counting, etc.) and other settings (distributed, etc.).
The lower bounds of Roddity and Virginia for their approach.

Pawel's papers on 4-cycle equivalence with some permutation problems or tree distance.

Lower bounds under Triangle Conjecture, such as dynamic and  the Enumeration classifications by Nofar Carmeli et al.

Mention reductions from triangle to $k$-cycles in other setting, like the fooling views paper by Abboud et al. 

Mention the hardness of approximation for diameter in distributed, as it also relies on not having small cycles.

Mention Chan's derandomization of the 3SUM to Conv3SUM reduction and say that it gives hope that all our results can be made deterministic too.

Mention the Duraj et al. paper (SODA 20) on equivalence between All-Edge Triangle and offline range query problems.

==> intro-or.tex <==

One of the most central and challenging goals in fine-grained complexity is to prove \emph{hardness of approximation} results for the many fundamental problems that we already know are hard to compute exactly.
With the exception of few results that follow from simple gadget reductions,\footnote{Similar to saying that the NP-hardness of $3$-coloring implies a $4/3-\eps$-hardness of approximation for the chromatic number.} understanding the time vs. approximation tradeoff seems to require specialized fine-grained \emph{gap amplification} techniques.
As we know from the quest for \emph{NP-hardness} of approximation that started in the early 90's, such techniques are not easy to come by, and the fine-grained restrictions on the reductions can only make matters worse.

Two notable success stories, highlighted in a recent survey by Rubinstein and Vassilevska Williams \cite{RVsurvey}, are the Distributed PCP framework \cite{ARW17} based on algebraic error-correcting codes, and a graph-products technique \cite{B+21} that has lead to impressive lower bounds for the Diameter problem \cite{DVVW19,Bonnet21a,Li21,DW21,Bonnet21b,DLV21}.
But we are still far away from satisfactory results for many problems (see the open questions in \cite{ARW17,RVsurvey}).
Even \emph{distance computations in graphs}, an extensively studied subject in fine-grained complexity, exhibits many huge gaps. 

As a case in point, consider the open questions below for three of the most basic problems in the area, each of them with a long list of upper bounds (summarized in Tables 1,2,3): distance oracles \cite{PR14,PRT12,3,4,5,6,7,8,9,10}, dynamic shortest paths \cite{1,2,3,4,5,6,7,8,9,10}, and the girth \cite{1,2,3,4,5,6,7,8,9,10}.


\begin{oq}
Can we preprocess a graph in $m^{1+o(1)}$ time and answer shortest path queries in $m^{o(1)}$ time with an $O(1)$-approximation? How about a much better, $3$-approximation?
\end{oq}

\begin{oq}
Can we preprocess a graph in $O(mn)$ time, then support edge-updates in $m^{o(1)}$ amortized time, and answer shortest path queries in $m^{o(1)}$ time with an $O(1)$-approximation? How about a $2$-approximation?
\end{oq}


\begin{oq}
Can we return an $O(1)$-approximation to the girth in $m^{1+o(1)}$ time? How about a $4/3$-approximation?
\end{oq}

The current upper bounds have the form of $O(k)$-approximation in $\tilde{O}(m^{1+1/k})$ time, meaning that only super-constant approximation factors are possible in $m^{1+o(1)}$ time.
It seems plausible that this is the right tradeoff, but it is hard to be confident without a hardness result. 
Such a tradeoff curve was recently broken, in an equally unexpected manner, for the Edit Distance problem \cite{BEGHS21,CDG+20,AN20}. 

Meanwhile, the lower bounds are consistent with positive answers to \emph{all} of these questions, even in \emph{weighted} graphs.\footnote{The case of \emph{directed} graphs is different however. For some of these problems even deciding if the distance is finite has strong lower bounds.}
Existing techniques cannot even rule out small (constant) approximation factors.

The barrier for proving higher lower bounds is common; it is the \emph{short cycle barrier} discussed below.
Overcoming this barrier is related to Open Question 5 in the distributed PCP paper \cite{ARW17} asking for gap amplification techniques from conjectures other than SETH.
This is because (the exact versions of) our distance computation problems are not SETH-hard; their hardness is via  reductions from (detecting or) \emph{listing triangles} in a graph, a problem that is hard under the 3SUM or APSP conjectures, but not SETH.



\paragraph{The Short Cycle Barrier.}
Suppose we are given a tripartite graph $G$ with parts $A,B,C$ and want to detect a triangle $a\in A, b \in B, c \in C$.\footnote{This tripartite version is equivalent to the general case by a standard reduction.}
Let $G'$ be the graph obtained from $G$ by removing the $B \times C$ edges.
For each pair $(b,c) \in E(G)$, what is the distance between $b$ and $c$ in $G'$?
It is $2$ if $(b,c)$ is in a triangle in $G$, and larger otherwise. 
But how much larger?
Unfortunately from a hardness of approximation perspective, the distance will probably not be more than $4$ due to a path with one \emph{zigzag}  $b \to a \to b' \to a' \to c$  that corresponds to a $5$-cycle in $G$ but not a triangle.
So we cannot go above $(2-\eps)$ factors in this way.

In FOCS 2010, P{\u{a}}tra{\c{s}}cu and Roditty \cite{PR14} devised an ingenious graph-products technique (that was an inspiration for the Diameter results \cite{B+21}) to push the lower bound beyond $2$.
The idea was to have a construction with $k$ layers such that a pair $b,c$ without a direct path (of length $k$) must make a zigzag in $k-1$ layers, making the distance $3k-2$.
Indeed, this was accomplished in a follow-up paper with Thorup \cite{PRT12} that went all the way up to $(3-\eps)$ factors, but it is clear that this is the limit of the approach. 

The natural and more promising approach for circumventing this barrier is to simply assume that there are no $\leq k$-cycles in the graph. 
Then, any effective zigzag must be \emph{long}, and even with the natural two-layered construction, would give us a lower bound of $\Omega(k)$.
Indeed, the distance for a pair $b,c$ would be $=2$ if the pair is in a triangle, versus $\geq k-1$ otherwise.
This would be reminiscent of the use of the girth conjecture in lower bounds for \emph{multiplicative} spanners \cite{PS89,Alt+93},
whereas the aforementioned graph-products technique is reminiscent of lower bounds for \emph{additive} spanners \cite{Woodruff06,AB17,ABP18}.\footnote{The Girth Conjecture and the techniques for additive spanners were already used, of course, for lower bounds against distance oracles as well. However, such lower bounds (and any information-theoretic arguments) cannot prove lower bounds higher than $m$; rather, they are interesting for understanding how much dense graphs can be compressed. Thus, the similarity can only be spiritual.}
All we have to do is to prove this gap amplification result for Triangle, amplifying the no-case from triangle-free to $\leq k$-cycle free.


\begin{oq}[Main Open Question]
\label{oq:main}
Can we prove hardness for finding a triangle in a $4$-cycle free graph? What if it is $k$-cycle free for all $k=O(1)$?
\end{oq}

Any progress on this question carries over to progress on the above questions, by the standard reductions.
But it is far from clear why such a gap amplification should be possible.
The needle-in-a-haystack flavor (and intuitive hardness) of triangle finding \emph{stems} from the possibility of a triangle hiding amidst plenty of $4$- or $5$-cycles.
In a $4$-cycle free graph no two nodes can have more than one common neighbor; doesn't that restrict the search space by too much?\footnote{Such high-girth assumptions can indeed reduce the complexity of some problems from almost-quadratic to almost-linear. In particular, in the Orthogonal Vectors problem with dimension $d=n^{o(1)}$ (at the core of the Diameter lower bounds, and many others), if no two vectors can have two coordinates that are non-zero, there is an $O(n d^2)$ algorithm.}

These contemplations touch upon a well-known hole in our understanding of graph problems. 
Indeed, by a simple reduction, proving such an amplification even if only for $k=4$ already resolves one of the most infamous open questions in fine-grained complexity:\footnote{By a simple trick where we subdivide a subset of the edges.}

\begin{oq}
Can we determine if a graph contains a $4$-cycle in $m^{1+o(1)}$ time?
\end{oq}

In 1994, Yuster and Zwick \cite{YZ97} put forth the conjecture that one cannot detect a $4$-cycle in a graph in subquadratic time. 
The longstanding upper bound is $O(m^{4/3})$ via a high-degree low-degree argument \cite{AYZ97}; it is at most $O(n^2)$ because when $m \geq 200\cdot n^{1.5}$ we can simply output ``yes'': by the Bondy-Simonovitz Theorem \cite{BS74}, a graph with such density must contain a $4$-cycle.
Frustratingly, to this date, the field of fine-grained complexity has not managed to show any hardness for this problem.
``\emph{What hope do we have to
understand more complex problems if we cannot settle the complexity of this simple one, even
conditionally?}''\footnote{This is a quote from the survey by Rubinstein and Vassilevska Williams \cite{RVsurvey} where it is referring to the approximability of the graph diameter problem. We find it no less poignant when considering the $4$-cycle problem.}

\subsection{Our Results}

In this paper we answer all of the above questions, some fully and some partially, under plausible hardness assumptions.
Our main contribution is a proof that triangle finding remains hard when the graph has very few short cycles. 

\begin{restatable}{theorem}{ThmRemovingCycles}[Removing Most $k$-Cycles]
\label{thm:main1}
Let $\eps',\eps>0$ and $k\geq 4$. Given a graph $G$ with maximum degree $\sqrt{n}$, for every $\alpha>0$, there is a randomized $O(n^{2-\eps})$-time algorithm that returns a subset of the edges $E' \subseteq E$ with an aswer to each edge $e\in E'$ to whether it participates in a triangle, and a set of $s=n^{3/2-3\alpha}$ subgraphs $G_1,\ldots,G_s$ such that:
\begin{itemize}
    \item If an edge $e \in E$ is in a triangle in $G$ then it is either in $E'$ or is in a triangle in one of the $G_i$'s.
    \item Each $G_i$ has $n^{1/2+\alpha}$ nodes of degree $n^{\alpha}$ with high probability, and contains only $O(n^{\frac{\omega-1}{4}+\eps'+k\alpha})$ $k$-cycles in expectation.
\end{itemize}
\end{restatable}

The problem of reporting which edges in a graph are in a triangle (All-Edge Triangle) is known to require $n^{2-o(1)}$ time, under the $3$-SUM Conjecture \cite{Pat10,KPP16} or under the APSP Conjecture~\cite{VX20}, and this holds even for graphs of degree $\sqrt{n}$.
Thus it is a very plausible conjecture that $n^{2-o(1)}$ is required.

Combining our new theorem with the standard reductions already resolves some of the hardness of approximation problems above. 
Each of the few remaining short cycles might result in a false positive, but since their number is small (and the degrees in the $G_i$ graphs are small), they can all be filtered in post-processing stage of subquadratic time.


\paragraph{Applications}
Our first corollary improves the $(3-\eps)$ hardness of P{\u{a}}tra{\c{s}}cu, Roditty, and Thorup \cite{PRT12} all the way up to $\omega(1)$ showing that $O(k)$-approximation with $\tilde{O}(m^{1+1/k})$ preprocessing is indeed the right tradeoff for distance oracles.\footnote{One caveat is that their lower bound is based on a set-intersection conjecture that rules out preprocessing with $m^{1+\eps}$ \emph{space} rather than \emph{time}, and is therefore stronger. On the other hand, our lower bound is based on the more popular 3SUM and APSP conjectures.}
Moreover, our lower bound applies to the easier \emph{offline} version of the problem where all the queries are given in advance.
 
\begin{corollary}[Hardness of Approximation for Offline Distance Oracles]
Assuming either the $3$-SUM or APSP Conjectures, no algorithm can return a $k$-approximation to the distance between $m$ pairs of nodes in a simple graph with $m$ edges in time $O(m^{1+1/4k-\eps})$\Atodo{todo}, where $\eps>0$.
\end{corollary}

The \emph{Subset Shortest Paths} problem in the above corollary is at the core of the dynamic shortest paths problem as well. 
By a straightforward reduction it implies that Chechik's decremental APSP $k$-approximation algorithm in total time $m^{1+1/ck}$\Atodo{todo} is tight up to the constant $c$.
For fully dynamic algorithms, we can strengthen the result further by ruling out algorithms that start with a cubic-time preprocessing phase (which is natural as it gives the algorithm enough time to precompute all the distances). However, in this fully dynamic case, the best known upper bound only achieves a $(\log{n})^k$-approximation in $m^{1+1/k}$ time.

\begin{corollary}[Hardness of Approximation for Dynamic APSP]
Assuming either the $3$-SUM or APSP Conjectures, no algorithm can preprocess a simple graph in $O(n^3)$ time and then support updates and queries in $O(m^{1/4k-\eps})$ time, for some $\eps>0$, where an answer to a query is a $k$-approximation to the distance between a given pair of nodes. \Atodo{todo: time bounds}
\end{corollary}

\Atodo{Not sure if it's better to include this third application or omit it. }
And as a third corollary, we show that any algorithm that obtains a $k$-approximate shortest cycle for each edge in the graph must spend $m^{1+1/ck}$ time.

\begin{corollary}[Hardness of Approximation for All-Edge Shortest Cycle]
Assuming either the $3$-SUM or APSP Conjectures, no algorithm can return a $k$-approximation to the shortest cycle that each edge is a part of in a simple graph with $m$ edges in time $O(m^{1+1/2k-\eps})$\Atodo{todo}, where $\eps>0$.
\end{corollary}

%This matches a very recent upper bound tradeoff for the girth. Alas, that algorithm does not solve the All-Edge version.


Let us now turn our attention back to the intriguing $4$-Cycle problem.
A direct corollary of our theorem is that the All-Edge version has a super-linear lower bound, finally extending the $m^{4/3}$ lower bound from P{\u{a}}tra{\c{s}}cu's seminal paper \cite{Pat10} for triangle enumeration to a hardness result for $4$-cycle enumeration.
If $\omega=2+o(1)$ the lower bound is $m^{5/4-o(1)}$.

\begin{restatable}[Hardness for $4$-Cycle Enumeration]{corollary}{CorEnum}\label{cor:Enum}
Assuming either the $3$-SUM or APSP Conjectures, no algorithm can process an $m$ edge graph in $O(m^{1+\frac{3-\omega}{2(4-\omega)}-\eps})$ time, for some $\eps>0$, and then enumerate $4$-cycles with $m^{o(1)}$ delay. \Atodo{it might make more sense to say this theorem for all $k \geq 4$ and change the text below.}
\end{restatable}

We can also derive super-linear $m^{1+1/ck}$ lower bounds for $k$-cycle enumeration for all $k$, from Theorem~\ref{thm:main1}. 
However, we can get a higher $m^{5/4-o(1)}$ lower bound by reducing from $4$-Cycle directly: 
simple gadget reductions prove that $k$-cycle (detection or enumeration) for any $k$ is at least as hard as hard as either the $k=3$ or $k=4$ case (see \cite{DKS17}).\footnote{The reduction simply subdivides some of the edges. Note that this trick is not useful in the hardness of approximation context because subdividing edges increases the distances even in the yes-case.} 
Either way, we separate $k$-cycle from the class $\textsc{DelayC}_{lin}$ of problems solvable with linear time preprocessing and constant delay. 
This class has received a lot of attention in recent years from the enumeration algorithms community (see e.g. \cite{1,2,3,4,5}).
Our result is somewhat surprising because enumerating all cycles (without restricting $k$) is \emph{in} the class $\textsc{DelayC}_{lin}$ \cite{sodapaper}.

\medskip
Theorem~\ref{thm:main1} does not fully resolve the Main Open Question~\ref{oq:main}, because it does leave $n^{\Omega(1)}$ short cycles in the graph.
This is not an issue for all of the applications above because the end-problem returns multiple answers (that can be filtered afterwards).
Unfortunately, this cannot be done for problems with a single output, such as our most basic $4$-Cycle detection problem.
Nonetheless, with a bit more work we can actually get rid of all $k$-cycles in the $k=4$ case.
 



%
%This matches a very recent upper bound tradeoff for the girth. Alas, that algorithm does not solve the All-Edge version.
%To prove a similar lower bound for the more basic girth problem, our gap amplification must get rid of \emph{all} $\leq k$-cycles.
%Unfortunately, Theorem~\ref{thm:main1} does leave $n^{\Omega(1)}$ short cycles (and therefore does not fully resolve the Main Open Question~\ref{oq:main}).
%Nonetheless, with a bit more work we can actually get rid of all $k$-cycles in the $k=4$ case.
%
%\Stodo{Something about this paragraph above doesn't feel incredibly good to me. Let's discuss when we meet. See also my second comment below.}

\paragraph{Removing \emph{all} $4$-Cycles}
Our most technical result is a strengthening of Theorem~\ref{thm:main1} in the $k=4$ case, giving a reduction to graphs that are \emph{completely} $4$-cycle free, finally establishing a conditional lower bound for $4$-Cycle.

\begin{restatable}{theorem}{ThmAllFourCycles}
\label{thm:main2}
Let $\eps>0$ and $0<\alpha<1/4-\frac{\omega-1}{8}-\eps/2$. Given a graph $G$ with maximum degree $\sqrt{n}$, there is a randomized $O(n^{2-\eps})$-time algorithm that returns a subset of the edges $E' \subseteq E$ with an answer for each $e\in E'$ to whether it participates in a triangle, and a set of $s=n^{3/2-3\alpha}$ subgraphs $G_1,\ldots,G_s$ such that:
\begin{itemize}
    \item If an edge $e \in E$ is in a triangle in $G$ then it is either in $E'$ or is in a triangle in one of the $G_i$'s.
    \item  With constant probability, each $G_i$ has $n^{1/2+\alpha}$ nodes of degree $n^{\alpha}$, and is $4$-cycle free.
\end{itemize}
\end{restatable}



\begin{restatable}[Hardness for $4$-Cycle Detection]{corollary}{CorFourDet}\label{cor:fourDet}
Assuming that triangle detection in graphs with maximum degree $\sqrt{n}$ requires $n^{2-o(1)}$ time, no algorithm can determine if an $m$-edge graph has a $4$-cycle in $O(m^{1+\frac{3-\omega}{2(5-\omega)}-\eps})$ time, for some $\eps>0$.
\end{restatable}


The longstanding upper bound for triangle detection is $O(\min\{m^{2\omega/(\omega+1)},n^{\omega}\})$, where $\omega\geq 2+o(1)$ is the fast matrix multiplication exponent \cite{YZ?}.
Even if an optimal matrix multiplication algorithm exists ($\omega=2$) no algorithm breaks the quadratic barrier when $m=n^{1.5}$.
This continues to be the case in the natural setting where the maximum degree (rather than the average degree) is $\sqrt{n}$.
Thus, breaking the hardness assumption at the base of our conditional lower bound would be a major breakthrough.
See Section~\ref{sec:discussion} for further discussion.

In fact, even for triangles, the 3SUM hardness from P{\u{a}}tra{\c{s}}cu's seminal paper \cite{Pat10} (and the later APSP hardness \cite{VX20}) are only known for the enumeration (or \emph{All-Edge} versions) but not for detection.
We show that the same kind of hardness carries over to $4$-cycle.

\begin{restatable}[Hardness for $4$-Cycle Enumeration]{corollary}{CorEnum}\label{cor:Enum}
Assuming either the $3$-SUM or APSP Conjectures, no algorithm can process an $m$ edge graph in $O(m^{1+\frac{3-\omega}{2(4-\omega)}-\eps})$ time, for some $\eps>0$, and then enumerate $4$-cycles with $m^{o(1)}$ delay.
\end{restatable}


\Stodo{Shouldn't we put this after Theorem 1.6? It follows from 1.6 already. To make the twist in the plot that you want for introducing the most technical result, instead of playing on the girth approx challenge, we can play on the 4-cycle detection and cycles classification challenge (with Unfortunately and then Nonetheless, to built it up in a similar way to what you are doing with the all-edge short cycle thing). Then, we add more consequences for girth approximation and hardness of Triangles in 4-cycle free graphs. To be honest I'm not completely sure about the all-edge short cycle problem.. it feels to me that we are selling it in a strange way as we compare it with an upper bound for an easier problem, computing the girth. If I understand correctly, you want to use it because it helps with this nice build up in the intro, which I feel we can do with 4-cycle detection and cycle classification challenge.}
\Atodo{I agree. That's a good idea. I was trying to keep the focus on approximation problems, but it's inevitable to break the focus at some point because we want to present the other results as well... I'll make the change soon.}
Gadget reductions prove that $k$-cycle (detection or enumeration) for any $k$ is at least as hard as hard as either the $k=3$ or $k=4$ case (see \cite{DKS17}). 
In the parlance of the enumeration algorithms literature, we separate $k$-cycle from the class $\textsc{DelayC}_{lin}$ of problems solvable with linear time preprocessing and constant delay.
This is somewhat surprising because enumerating all cycles (without restricting $k$) is in $\textsc{DelayC}_{lin}$ \cite{sodapaper}.

The lower bound for $4$-Cycle follows from the following corollary, giving a positive answer to the $k=4$ case in the Main Open Question~\ref{oq:main}.


\begin{restatable}[Hardness for Triangle in $4$-Cycle-Free Graphs]{corollary}{CorFourFree}\label{cor:fourFree}
Assuming that triangle detection in graphs with degree $\sqrt{n}$ requires $n^{2-o(1)}$ time, no algorithm can determine if an $m$-edge $4$-cycle free graph has a triangle in $O(m^{1+\frac{3-\omega}{2(5-\omega)}-\eps})$ time, for some $\eps>0$.
\end{restatable}


Consequently, we improve the lower bound for the basic girth approximation problem from $4/3-\eps$ to $5/3-\eps$. 

\subsection{Related Work}

The approximating APSP without scaling paper, and Zwick's $(1+\eps)$-APSP. It's worth discussing other approximation results for APSP such as DHZ.

Other hardness of approximation results in P, e.g. for directed shortest cycle by Mina and Virginia \cite{DV21}, and the results that follow from Distributed PCPs. Maybe also the approximate counting results by Dell et al.

Other hardness of approximation for distance computation problems, and other open questions, e.g. $(1+\eps)$ dynamic APSPS in planar.

Lower bounds for $4$-cycle in other settings (directed, counting, etc.) and other settings (distributed, etc.).
The lower bounds of Roddity and Virginia for their approach.

Pawel's papers on 4-cycle equivalence with some permutation problems or tree distance.

Lower bounds under Triangle Conjecture, such as dynamic and  the Enumeration classifications by Nofar Carmeli et al.

Mention reductions from triangle to $k$-cycles in other setting, like the fooling views paper by Abboud et al. 

Mention the hardness of approximation for diameter in distributed, as it also relies on not having small cycles.

Mention Chan's derandomization of the 3SUM to Conv3SUM reduction and say that it gives hope that all our results can be made deterministic too.

Mention the Duraj et al. paper (SODA 20) on equivalence between All-Edge Triangle and offline range query problems.

==> older-intro.tex <==

\section{Introduction - new}

The main result of this paper is the first conditional hardness result for $4$-cycle detection showing that a fast enough algorithm implies a breakthrough for triangle-detection as well. 

\begin{theorem}
\label{thm:main}
For all $\eps>0$ there is a $\delta>0$ such that if $4$-cycle detection on $m$ edge graphs can be solved in $O(m^{1.1-\eps})$ time, then triangle-detection in graphs with maximum degree $\sqrt{n}$ can be solved in $O(n^{2-\delta})$ time.
\end{theorem}

None of the existing techniques is capable of breaking the $n^2$ barrier for triangle detection when $m=n^{1.5}$ and this is even assuming that $\omega=2$. 
This is still the case when the graph is assumed to be regular with degrees $\sqrt{n}$, thus motivating the following more concrete version of the triangle conjecture (see Section~\ref{sec:discussion} on the relationship between the two conjectures).

\begin{conjecture}[The Regular Triangle Conjecture]
Triangle-detection in $\sqrt{n}$-regular graphs requires $n^{2-o(1)}$ time.
\end{conjecture}



\subsection{Approximations}

Open question: what is the best approximation factor for the girth in $m^{1+o(1)}$ time?

The current best upper bound has the form $k$-approximation in $m^{1+1/k}$ time.

The previous lower bounds are:
\begin{enumerate}
\item  $1.33-\eps$ because $3$ vs. $4$ assuming Triangle Conjecture. 
\item $1.5-\eps$ if we also assume the $4$-Cycle Conjecture, because then $4$ vs. $6$ is hard. 
\end{enumerate}

From our main result we already get the $1.5-\eps$ lower bound while only assuming the hardness of Triangle (in regular graphs).
By tweaking the reduction a bit, we can prove an even higher lower bound of $1.66-\eps$: it is hard to find a triangle even in a graph that is $4$-cycle free; i.e. $3$ vs. $5$ is hard.


\begin{theorem}
\label{thm:main}
For all $\eps>0$ there is a $\delta>0$ such that if triangle detection on $m$ edge graphs that are $4$-cycle free can be solved in $O(m^{1.1-\eps})$ time, then triangle-detection in graphs with maximum degree $\sqrt{n}$ can be solved in $O(n^{2-\delta})$ time.
\end{theorem}

\begin{corollary}
There is no $1.66-\eps$ approximation for the girth in $m^{1+o(1)}$ time, assuming the Regular Triangle Conjecture.
\end{corollary}

This result partially resolves a conjecture by Roditty and Vassilevska Williams.

For enumeration problems our results are \emph{much} stronger. 
We can rule out any constant factor approximation in $m^{1+o(1)}$ time, and in fact our lower bound tradeoff almost matches the upper bound (that only works for detection as far as we're aware).
We state our lower bound for the most basic version of the enumeration problem.

\begin{theorem}
\label{thm:main}
If we can return a $k$-approximation to the shortest cycle that passes through each node in a graph in $O(m^{1+1/(2k-2)-\eps})$ time, then the 3SUM and APSP conjectures are false.
\end{theorem}

\paragraph{Remark.} All of our lower bounds are parameterized by a certain parameter $\delta>0$. We can only prove our results for $\delta=1/4-0.01$ but it is plausible that a deeper combinatorial understanding will lead to $\delta \to 0$. In this case, our lower bounds for detection go up from $m^{1.1}$ and our lower bound for $k$-approximate listing exactly matches the $m^{1+1/k}$ upper bound (for detection). This means that breaking the recent $m^{1+1/k}$ bound will either require an algorithm that inherently cannot solve the (basic) listing problem, or it would refute certain plausible combinatorial assumptions.


\subsection{Classification}

\begin{theorem}[Alon-Yuster-Zwick]
If $H$ is a forest then the $H$-detection problem can be solved in $\tilde{O}(m)$ time.
\end{theorem}


\begin{theorem}[Dahlgaard-Knudsen-Stockel]
For all integer $k\geq 3$, if $k$-Cycle-detection problem has a $T(m)$ time algorithm, then either $C_3$-detection or $C_4$-detection can be solved in $T(O(m))$ time.
\end{theorem}

\begin{corollary}
If $H$ is a forest, then the $H$-detection problem can be solved in $\tilde{O}(m)$ time.
Otherwise, there is a subgraph $H'$ of $H$ such that the $H'$-detection problem requires $m^{1.1-o(1)}$ time, assuming the Regular Triangle Conjecture.
\end{corollary}

\begin{corollary}
If $H$ is a forest, then the $H$-enumeration problem can be solved in $\tilde{O}(m)$ time preprocessing and constant delay.
Otherwise, there is a subgraph $H'$ of $H$ such that the $H'$-enumeration problem cannot be solved with $O(m^{1.1-\eps})$ preprocessing time and $n^{\eps}$ delay, assuming either the 3SUM or the APSP conjectures.
\end{corollary}


\subsection{The Strong Zero Triangle Conjecture}

Finally, we turn our attention to the first question: can we base the hardness of Triangle and $4$-Cycle (detection) on one of the central conjectures of fine-grained complexity?
We also make progress towards this goal by proving the Regular Triangle Conjecture (and therefore also all the conditional lower bounds above) assuming the hardness of a variant of the Zero-Triangle problem.

\begin{definition}[Zero-Triangle]
Given a tripartite graph $G=(A\times B\times C,E)$ with integral edge weights $w:E \to [-W,+W]$ decide if there is a triangle $(a,b,c)\in A \times B \times C$ with total weight $w(a,b)+w(b,c)+w(a,c)=0$.
\end{definition}

Ignoring subpolynomial improvements, there are only two algorithms for this problem.
The first is a brute force over all triples and its running time is $|A|\cdot |B| \cdot |C|$.
In the symmetric setting where $|A|=|B|=|C|=n/3$ this is $O(n^3)$ and it is optimal under both $3$-SUM and APSP conjectures, as long as $W=\Omega(n^3)$. 
The second algorithm is faster when $W$ is small enough. It applies the standard exponentiation trick (encoding $w$ with $2^w$) to reduce summation to multiplication and then uses fast matrix multiplication. In the symmetric setting the running time is $O(W \cdot n^\omega)$ and otherwise it is a complicated expression that depends on the rectangular matrix multiplication exponent.
Assuming $\omega=2$ the upper bound simplifies to ***.
It is natural to conjecture that this bound cannot be broken for Zero-Triangle.

\begin{conjecture}[The Strong Zero-Triangle Conjecture]
Zero-Triangle requires *** time. 
\end{conjecture}

While this conjecture is not known to be implied by the $3$-SUM and APSP conjectures (see Section~\ref{sec:discussion} for a discussion) its plausibility has the same source.
In fact, it is analogous to the stronger version of the APSP conjecture recently studied by Chan, Vassilevska, and Xu \cite{CVX}.
Notably, this is a problem that is hard due to the weights and the addition operator and \emph{not} due to the graph structure: the input graph may be assumed to be complete.
Thus, we find it surprising that it explains the hardness of our purely structural subgraph detection problems; in particular it gives a \emph{tight} lower bound for Triangle.

\begin{theorem}
If the Regular Triangle Conjecture is false, then Zero-Triangle with $|A|=n,|B|=|C|=\sqrt{n}$ and $W=\sqrt{n}$ can be solved in $O(n^{2-\eps})$ time, for some $\eps>0$, and the Strong Zero Triangle Conjecture is false.
\end{theorem}

The reduction is rather simple but we find the statement quite interesting.
First, it bases the Regular Triangle Conjecture (and the entire classification of the subgraph detection problem) on a hardness assumption of a very different nature.
Second, it makes a substantial step towards establishing the Triangle and $4$-Cycle Conjectures under the more central $3$-SUM or APSP Conjectures.
And third, assuming $\omega=2$, it pinpoints the challenge that one must resolve before making any further progress on Triangle, since the lower bound is completely tight for all density regimes (see Section~\ref{sec:discussion}).  


\section{Introduction - old}

Arguably the two simplest graph problems without near-linear time algorithms are Triangle and $4$-Cycle: Does a given graph contain a triangle as a subgraph? Does it contain a $4$-cycle?
We are in the most basic setting of simple graphs on $n$ nodes and $m$ edges where a subgraph is obtained by deleting nodes and edges.\footnote{Sometimes called the not-necessarily induced case.}

The longstanding upper bounds are $O(\min\{m^{4/3},n^2 \})$ for $4$-Cycle, and $O(\min\{m^{2\omega/(\omega+1)},n^{\omega}\})$ for Triangle, where $\omega\geq 2$ is the fast matrix multiplication exponent.
Under the popular assumption that $\omega=2$, the bounds coincide at $O(\min\{m^{4/3},n^2 \})$.
These bounds are achieved with neat and simple arguments. A high-degree low-degree strategy reduces the problem to two cases: either one of the nodes of the triangle has degree $\leq m^{1/3}$ or all three nodes have degree $>m^{1/3}$ -- but there can only be $m^{2/3}$ such nodes. 
In the first case, an exhaustive search over the neighborhoods of low-degree nodes suffices, and in the latter case we use fast matrix multiplication on a smaller dense graph.
The $4$-cycle algorithm is similar with one interesting difference: in the dense case we can simply output ``yes'' without using fast matrix multiplication because, by the Bondy-Simonovitz Theorem, a graph with average degree above $10\sqrt{n}$ must have a $4$-cycle.

It is reasonable to believe that $\Omega(\min\{m^{4/3},n^2\})$ is also a lower bound. 
This was suggested in 1999 for $4$-Cycle by Yuster and Zwick, and in 2014 for Triangle by Abboud and Vassilevska Williams (where it was used as the basis of conditional lower bounds for dynamic problems). 
But it is far from clear that these conjectures are true, not even in their relaxed form:

\begin{conjecture}[The Weak Triangle Conjecture]
Triangle-detection cannot be solved in $\tilde{O}(m)$ time.
\end{conjecture}

\begin{conjecture}[The Weak $4$-Cycle Conjecture]
$4$-Cycle-detection cannot be solved in $\tilde{O}(m)$ time.
\end{conjecture}



Stirred by the thought ``\emph{What hope do we have to
understand more complex problems if we cannot settle the complexity of this simple one, even
conditionally?}''\footnote{This is a quote from the survey by Rubinstein and Vassilevska Williams \cite{SETHvsApx} where it is referring to the graph diameter problem. We find it no less poignant when considering Triangle and $4$-Cycle.}
the goal of this paper is to investigate the two most natural questions from the perspective of fine-grained complexity:

\begin{enumerate}
    \item Can we justify these conjectures under other hardness assumptions? Ideally we would prove them under a one of the central conjectures from fine-grained complexity such as 3SUM, APSP, or SETH.
    \item Can we reduce these problems to one another? In particular, it is desirable to reduce (the seemingly harder) Triangle to $4$-Cycle.
\end{enumerate}

These are notoriously difficult open problems in fine-grained complexity. 
Ever since Patrascu's \cite{Pat10} 3SUM-hardness result for triangle \emph{enumeration}, in the early days of this field, researchers have been trying to get any lower bound for the more basic \emph{detection} problem.
And the situation is even worse for $4$-cycle detection since no previous work has managed to reduce any natural and difficult-looking problem to $4$-Cycle, not even Triangle,\footnote{On the other hand, triangle detection is known to be harder than certain batched versions of set intersection. Moreover, if one makes the ``combinatorial only'' restriction, triangle detection is known to be harder than Boolean Matrix Multiplication.} and even the enumeration version is not known to be conditionally hard.
Still, we find these questions too important to let go of; not only for the sake of our two specific intriguing problems, but as we discuss next, also for the sake of the subgraph detection problem in its full generality. 

\subsection{Which Graph Patterns Can be Found in Linear Time?}

The problem of finding a certain small pattern in a large input graph is fundamental.
It is the core problem of the \emph{Data Mining} field, with a wide-ranging set of applications that spread across every topic within computer science.
Its most basic form is the following.

\begin{definition}[The $H$-detection problem]
Does a given simple graph $G$ contain the graph $H$ as a subgraph? 
\end{definition}

For example, Triangle is $C_3$-detection and $4$-Cycle is $C_4$-detection.
The pattern $H$ is treated as having a constant size, independent of the size of $G$.
%$k$ and the input graph $G$ has $n \gg k$ nodes and $m$ edges.
%We do not require the subgraph to be \emph{induced}, so e.g. a complete graph on $n\geq 3$ nodes does contain a triangle, and we do not allow contracting edges, so e.g. a single edge does not contain a $4$-cycle.
%This is arguably the most natural setting.
The complexity of this problem has been investigated extensively in every popular computational model, e.g. circuits \cite{1,2,3}, query complexity \cite{1,2,3}, property testing \cite{1,2,3}, quantum \cite{1,2,3}, distributed \cite{1,2,3}, dynamic \cite{1,2,3}, and parallel \cite{1,2,3}. 
In this paper we are interested in the most standard setting of worst case time complexity (in the Word-RAM with randomness).


Whereas traditional complexity theory equates efficiency with polynomial running time, the ethos of the more-modern fine-grained complexity is that ``efficient'' equals \emph{near-linear} time.
This is motivated by the ever growing sizes of data.
So rather than classifying the problems into the P and NP-hard classes, the first-order question is whether a problem can be solved in $\tilde{O}(m)$ time or not.\footnote{The $\tilde{O}(\cdot)$ notation hides polylogarithmic factors.} 
From this perspective, the main question in this context is the following.

\medskip
\begin{center}
\textbf{Main Question:}
\emph{For which patterns $H$ can the $H$-detection problem be solved in $\tilde{O}(m)$ time?}

\end{center}

At first sight it might seem that only trivial patterns like a star graph can be detected in linear time. 
However, the 1994 \emph{color-coding} technique \cite{AYZ} of Alon, Yuster, and Zwick enables us to detect even interesting patterns like $k$-path or $k$-matching in near-linear time. 
In fact, any \emph{acyclic} pattern can be detected efficiently. 

\begin{theorem}[\cite{AYZ}]
If $H$ is a forest then the $H$-detection problem can be solved in $\tilde{O}(m)$ time.
\end{theorem}

It is natural to conjecture that these are the \emph{only} patterns that can be detected in near-linear time.
Even for the two simplest cyclic patterns -- triangle and $4$-cycle -- no near-linear time algorithm is known to date.
Indeed, simple gadget reductions prove that one must solve either $C_3$-detection or $C_4$-detection in near-linear time in order to solve any other cyclic subgraph detection in near-linear time.\footnote{At a high level, this can be proved as follows. If $H$ is cyclic then it contains some $C_k$ as a subgraph, and therefore $H$-detection is harder than $C_k$-detection. Then, to reduce $C_3$ or $C_4$ to the $C_k$ case with $k>4$, we subdivide a subset of the edges (carefully chosen via color-coding) such that a short cycle becomes a longer cycle.}

\begin{theorem}[?]
If $H$ is not a forest and the $H$-detection problem has an $\tilde{O}(m)$ time algorithm, then either $C_3$-detection or $C_4$-detection can be solved in $\tilde{O}(m)$ time.
\end{theorem}

In the parlance of fine-grained complexity, the main question is settled if one assumes \emph{two} conjectures: the Weak Triangle Conjecture \emph{and} the Weak $4$-Cycle Conjecture.  
This adds more motivation to the two natural but difficult open questions above:
\begin{enumerate}
    \item Can we resolve the main question under other conjectures from fine-grained complexity?
    \item Can we reduce the number of conjectures needed to resolve the main question down to one? 
\end{enumerate}

%These are notoriously difficult open problems in fine-grained complexity. 
%Ever since Patrascu's \cite{Pat10} 3SUM-hardness result for triangle \emph{enumeration}, in the early days of this field, researchers have been trying to get any lower bound for the more basic \emph{detection} problem.
%And the situation is even worse for $4$-cycle detection since no previous work has managed to reduce any natural and difficult-looking problem to $4$-cycle detection, not even triangle-detection.\footnote{On the other hand, triangle detection is known to be harder than certain batched versions of set intersection. Moreover, if one makes the ``combinatorial only'' restriction, triangle detection is known to be harder than Boolean Matrix Multiplication.}
%Still, these questions are too important to let go of: if we do not understand what are arguably the simplest natural problems, what hope do we have of reaching the final goals of complexity theory?
%We view this paper as making major progress towards resolving both of them.


\subsection{Results}

The main result of this paper is the first conditional hardness result for $4$-cycle detection showing that a fast enough algorithm implies a breakthrough for triangle-detection as well. 

\begin{theorem}
\label{thm:main}
For all $\eps>0$ there is a $\delta>0$ such that if $4$-cycle detection on $m$ edge graphs can be solved in $O(m^{5/4-\eps})$ time, then triangle-detection in graphs with maximum degree $\sqrt{n}$ can be solved in $O(n^{2-\delta})$ time.
\end{theorem}

None of the existing techniques is capable of breaking the $n^2$ barrier for triangle detection when $m=n^{1.5}$ and this is even assuming that $\omega=2$. 
This is still the case when the graph is assumed to be regular with degrees $\sqrt{n}$, thus motivating the following more concrete version of the triangle conjecture (see Section~\ref{sec:discussion} on the relationship between the two conjectures).

\begin{conjecture}[The Regular Triangle Conjecture]
Triangle-detection in $\sqrt{n}$-regular graphs requires $n^{2-o(1)}$ time.
\end{conjecture}

From this conjecture and the new reduction it follows that $m^{5/4-o(1)}$ time is required for $4$-cycle detection \emph{and} for the detection of any cyclic subgraph.
Thus, the full classification asked by the main question can now be based on this single natural conjecture about triangle detection.

\begin{corollary}
The time complexity of the $H$-detection problem is:
\begin{itemize}
    \item $\tilde{O}(m)$ if $H$ is a forest, and
    \item $m^{5/4-o(1)}$ if $H$ is not a forest, assuming the Regular Triangle Conjecture.
\end{itemize}
\end{corollary}

Our new reduction makes substantial progress towards the goal of reducing the number of conjectures down to one (the second open questions above).
Along the way (using a subset of the ideas) we are finally able to extend Patrascu's \cite{Pat10} $3$-SUM lower bound for triangle \emph{enumeration} to $4$-cycle enumeration.
Patrascu's result was recently strengthened by Vassilvska Williams and Xu \cite{VX} such that it is based on \emph{both} the $3$-SUM and APSP conjectures; this now also holds for the simpler looking $4$-cycle enumeration problem.

\begin{theorem}
If for some $\eps>0$ there is an algorithm that can preprocess a graph in $O(m^{4/3-\eps})$ time and then enumerates $4$-cycles with $n^{o(1)}$ delay, then the Zero Triangle problem can be solved in truly-subcubic time, and the $3$-SUM and APSP Conjectures are false.
\end{theorem}

Finally, we turn our attention to the first question: can we base the hardness of Triangle and $4$-Cycle (detection) on one of the central conjectures of fine-grained complexity?
We also make progress towards this goal by proving the Regular Triangle Conjecture (and therefore also all the conditional lower bounds above) assuming the hardness of a variant of the Zero-Triangle problem.

\begin{definition}[Zero-Triangle]
Given a tripartite graph $G=(A\times B\times C,E)$ with integral edge weights $w:E \to [-W,+W]$ decide if there is a triangle $(a,b,c)\in A \times B \times C$ with total weight $w(a,b)+w(b,c)+w(a,c)=0$.
\end{definition}

Ignoring subpolynomial improvements, there are only two algorithms for this problem.
The first is a brute force over all triples and its running time is $|A|\cdot |B| \cdot |C|$.
In the symmetric setting where $|A|=|B|=|C|=n/3$ this is $O(n^3)$ and it is optimal under both $3$-SUM and APSP conjectures, as long as $W=\Omega(n^3)$. 
The second algorithm is faster when $W$ is small enough. It applies the standard exponentiation trick (encoding $w$ with $2^w$) to reduce summation to multiplication and then uses fast matrix multiplication. In the symmetric setting the running time is $O(W \cdot n^\omega)$ and otherwise it is a complicated expression that depends on the rectangular matrix multiplication exponent.
Assuming $\omega=2$ the upper bound simplifies to ***.
It is natural to conjecture that this bound cannot be broken for Zero-Triangle.

\begin{conjecture}[The Strong Zero-Triangle Conjecture]
Zero-Triangle requires *** time. 
\end{conjecture}

While this conjecture is not known to be implied by the $3$-SUM and APSP conjectures (see Section~\ref{sec:discussion} for a discussion) its plausibility has the same source.
In fact, it is analogous to the stronger version of the APSP conjecture recently studied by Chan, Vassilevska, and Xu \cite{CVX}.
Notably, this is a problem that is hard due to the weights and the addition operator and \emph{not} due to the graph structure: the input graph may be assumed to be complete.
Thus, we find it surprising that it explains the hardness of our purely structural subgraph detection problems; in particular it gives a \emph{tight} lower bound for Triangle.

\begin{theorem}
If the Regular Triangle Conjecture is false, then Zero-Triangle with $|A|=n,|B|=|C|=\sqrt{n}$ and $W=\sqrt{n}$ can be solved in $O(n^{2-\eps})$ time, for some $\eps>0$, and the Strong Zero Triangle Conjecture is false.
\end{theorem}

The reduction is rather simple but we find the statement quite interesting.
First, it bases the Regular Triangle Conjecture (and the entire classification of the subgraph detection problem) on a hardness assumption of a very different nature.
Second, it makes a substantial step towards establishing the Triangle and $4$-Cycle Conjectures under the more central $3$-SUM or APSP Conjectures.
And third, assuming $\omega=2$, it pinpoints the challenge that one must resolve before making any further progress on Triangle, since the lower bound is completely tight for all density regimes (see Section~\ref{sec:discussion}).  

\subsection{Related Work}

==> tables.tex <==
\begin{figure}
\centering
\begin{tabular}{|c || p{70pt} | p{100pt} | p{95pt} | p{40pt} |} 
 \hline
 \textbf{Problem} & \textbf{Multiplicative Approx.} & \textbf{Upper Bound} & \textbf{Lower Bound} & \textbf{Citation} \\ [0.5ex] 
  \hline
 \hline
 \textbf{Decremental APSP} & $1$ & $O(mn^2)$ total update time, $\tilde{O}(1)$ query &  & \cite{shiloach1981line} \\
     \hline
  & $1+\varepsilon$ & $\tilde{O}(mn)$ time, $\tilde{O}(1)$ query &  & \cite{roditty2012dynamic} \\
    \hline
  & $2k-1+\varepsilon$ & $\tilde{O}(n^{2+1/k+o(1)})$ time, $\tilde{O}(1)$ query &  & \cite{bernstein2011improved} \\
    \hline
  & $(2+\varepsilon)^k - 1$ & $O(m^{1+1/k+o(1)})$ time, $\tilde{O}(1)$ query &  & \cite{henzinger2014decremental} \\
  \hline
  & $(2+\varepsilon)k-1$ & $O(mn^{1/k+o(1)})$ time, $\tilde{O}(1)$ query &  & \cite{chechik2018near} \\
      \hline
  & $2-\varepsilon$ &  &  $\Omega(mn^{1-\varepsilon})$ time if $\tilde{O}(1)$ query, assuming OMv & \cite{henzinger2015unifying} \\
  \hline
 \hline
 \textbf{Full APSP} & $1$ & $\tilde{O}(n^2)$ update &  & \cite{demetrescu2004new} \\
     \hline
  & $2+\varepsilon$ & $\tilde{O}(m^{1+o(1)})$ update&  & \cite{bernstein2009fully} \\
    \hline
  & $4k$ & $\tilde{O}(n^{1+1/k+o(1)})$ update &  & \cite{baswana2012fully} \\
    \hline
  & $(\log n)^{O(k)}$ & $\tilde{O}(n^{1/k})$ update &  & \cite{forster2021dynamic} \\
      \hline
  & $2-\varepsilon$ &  &  $\Omega(mn^{1-\varepsilon})$ time if $\tilde{O}(1)$ query, assuming OMv & \cite{henzinger2015unifying} \\
  [1ex] 
 \hline
\end{tabular}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{|c || p{70pt} | p{100pt} | p{95pt} | p{40pt} |} 
 \hline
 \textbf{Problem} & \textbf{Multiplicative Approx.} & \textbf{Upper Bound} & \textbf{Lower Bound} & \textbf{Citation} \\ [0.5ex] 
  \hline
 \hline
 \textbf{Distance Oracle} & $1$ & $O(nm)$ precprocessing time, $O(n^2)$ space, $O(1)$ query &  & \cite{thorup1999undirected} \\
%  \hline
%  & $1$ & $O(1)$ prep., $O(1)$ space, $O(m)$ query &  & \cite{thorup1999undirected} \\
    \hline
  & $2$ & $\tilde{O}(m^{1/2}n^{3/2})$ prep., $O(n^2)$ space, $O(1)$ query &  & \cite{cohen2001all} \\
      \hline
  & $7/3$ & $\tilde{O}(n^{7/3})$ prep., $O(n^2)$ space, $O(1)$ query &  & \cite{cohen2001all} \\
      \hline
  & $3$ & $\tilde{O}(n^{2})$ prep., $O(n^2)$ space, $O(1)$ query &  & \cite{cohen2001all} \\
        \hline
  & $3$ & $\tilde{O}(m^{2/3}n)$ prep., $O(n^{5/3})$ space, $O(1)$ query &  & \cite{dor2000all} \\
        \hline
  & $64k$ & $\tilde{O}(mn^{1/k})$ prep., $\tilde{O}(n^{1+1/k})$ space, $\tilde{O}(n^{1/k})$ query &  & \cite{awerbuch1998near} \\
        \hline
  & $2k+\varepsilon$ & $\tilde{O}(mn^{1/k})$ prep., $\tilde{O}(n^{1+1/k})$ space, $\tilde{O}(n^{1/k})$ query &  & \cite{cohen1998fast} \\
        \hline
  & $2k-1$ & $\tilde{O}(mn^{1/k})$ prep., $\tilde{O}(n^{1+1/k})$ space, $\tilde{O}(1)$ query &  & \cite{thorup2005approximate} \\
          \hline
  & $2k-1$ & $\tilde{O}(n^2)$ prep., $\tilde{O}(n^{1+1/k})$ space, $\tilde{O}(1)$ query &  & \cite{thorup2005approximate} \\
          \hline
  & $11$ & $\tilde{O}(m+n^{23/12})$ prep., $\tilde{O}(n^{3/2})$ space, $\tilde{O}(1)$ query &  & \cite{baswana2008distance} \\
            \hline
  & 2-\varepsilon &  & $\tilde{\Omega}(n^2)$ space and prep. if query in~$O(1)$, assuming SetIntersection & \cite{PR14} \\
  \hline
  & 3-\varepsilon &  & $\tilde{\Omega}(m^{1+\Omega(1)})$ space and prep. if query in~$O(1)$, assuming SetIntersection & \cite{PRT12} \\
  \hline
  & O(1) &  & $\tilde{\Omega}(n^{1+\Omega(1)})$ space and prep. if query in~$O(1)$, even for $m=\tilde{O}(n)$, cell probe & \cite{sommer2009distance} \\
 \hline
 \hline
 \textbf{Girth (undirected)} & $1$ & $O(nm),\; O(n^\omega)$ &  & \cite{itai1978finding} \\
  \hline
  & 1 & & $\Omega(n^{3-\varepsilon})$ for combinatorial assuming APSP/BMM & \cite{williams2018subcubic} \\
 \hline
  & $4/3$ & $O(n^2)$ &  & \cite{itai1978finding} \\  
   \hline
  & $2$ & $\tilde{O}(n^{5/3})$ &  & \cite{roditty2012subquadratic} \\  
  \hline
   & $8/3$ & $\tilde{O}(n^{3/2})$ &  & \cite{lingas2008efficient} \\  
   \hline
  & $2^k,\; k\geq 2$ & $\tilde{O}(n^{1+1/k})$ &  & \cite{dahlgaard2017new} \\ 
      \hline
  & $4/3 - \varepsilon$ &  & $\Omega(m^{1+\omega(1)})$ assuming Triangle & folklore \\  
  %  \hline
  %& $5/3 - \varepsilon$ &  & $\Omega(m^{1+\omega(1)})$ assuming Regular-Triangle & \textbf{this paper} \\  
  [1ex] 
 \hline
\end{tabular}
\end{figure}
